ROSE: Transformer-Based Refactoring Recommendation for Architectural Smells

Architectural smells such as God Class, Cyclic Dependency, and Hub-like Dependency degrade software quality and maintainability. Existing tools detect such smells but rarely suggest how to fix them. This paper explores the use of pre-trained transformer models--CodeBERT and CodeT5--for recommending suitable refactorings based on detected smells. We frame the task as a three-class classification problem and fine-tune both models on over 2 million refactoring instances mined from 11,149 open-source Java projects. CodeT5 achieves 96.9% accuracy and 95.2% F1, outperforming CodeBERT and traditional baselines. Our results show that transformer-based models can effectively bridge the gap between smell detection and actionable repair, laying the foundation for future refactoring recommendation systems. We release all code, models, and data under an open license to support reproducibility and further research.

==> 6-conclusion.tex <==
\section{Conclusion and Future Work}
\label{sec:Conclusion}
%\PN{I am going to revise this section.}
%This thesis investigated the 
In this paper, we conceived \RS, a  Transformer-based model for recommending software refactoring types based on source code. The study focused on three common refactorings, \ie \textit{Extract Method}, \textit{Move Class}, and \textit{Pull Up Method}, each of which is related to well-known architectural smells such as God Class and Cyclic Dependency. %The primary objective was to evaluate the performance of two state-of-the-art pre-trained models—CodeBERT and CodeT5—in distinguishing these refactoring patterns from labeled code fragments.

\begin{comment}
To this end, a curated dataset of real-world Java code was processed and tokenized using sliding window techniques to accommodate longer input sequences. Each model was fine-tuned using Hugging Face’s Trainer API, and evaluated over multiple training configurations. Key performance metrics—accuracy, F1-score, precision, and recall—were tracked and compared across 10 epochs.
\end{comment}

The results showed that CodeT5 consistently outperforms CodeBERT in all metrics, achieving a maximum validation accuracy of 96. 98\% and a F1 score of 0.9516 in Epoch 9. In contrast, CodeBERT reaches a maximum accuracy of 85.28\% and F1-score of 0.8527. Confusion matrix analysis revealed that both models struggled with the \textit{Extract Method} class due to its similarity with \textit{Move Class}, but performed well on \textit{Pull Up Method}. CodeT5 demonstrated stronger generalization capabilities and faster convergence, while CodeBERT showed signs of overfitting in later epochs.
These findings confirm the viability of using pre-trained Transformer models--especially encoder–decoder architectures like CodeT5--for automated software refactoring support. Such models can complement traditional static analysis by offering intelligent, data-driven insights into code structure and quality.

We anticipate that there are various future research directions as follows. 
Some code fragments may involve more than one refactoring; future work could explore models that support multi-label outputs. Moreover, incorporating attention visualization or saliency maps could help explain why the model chooses a particular refactoring class, increasing trust and usability. Finally, larger variants (e.g. CodeT5-Large or CodeGen) could be evaluated to see whether they yield higher accuracy and F1-scores on more complex refactorings.


\begin{comment}
Several promising directions remain for further investigation:

\begin{itemize}
    \item \textbf{Multi-label classification:} Some code fragments may involve more than one refactoring; future work could explore models that support multi-label outputs.
    
    \item \textbf{Explainability:} Incorporating attention visualization or saliency maps could help explain why the model chooses a particular refactoring class, increasing trust and usability.
    
    \item \textbf{Model scaling:} Larger models like CodeT5-Large or CodeGen could be evaluated for their ability to improve performance on more complex refactorings.
    
    \item \textbf{Real-time integration:} Embedding this classifier in IDEs could provide refactoring suggestions during development, enabling just-in-time code improvements.
    
    \item \textbf{Expanded datasets:} Leveraging more diverse codebases and programming languages could improve model robustness and generalizability across software domains.
    
    \item \textbf{Refactoring generation:} Extending this work from classification to actual transformation of code (i.e., applying the predicted refactoring) would be a natural next step.
\end{itemize}


In conclusion, this research presents an effective and scalable approach to refactoring type prediction using Transformer-based architectures, with strong potential for integration into modern software engineering workflows.
\end{comment}
